Mini-Splatting: Representing Scenes with a Constrained Number of Gaussians

In this study, we explore the challenge of efficiently representing scenes with a constrained number of Gaussians. Our analysis shifts from traditional graphics and 2D computer vision to the perspective of point clouds, highlighting the inefficient spatial distribution of Gaussian representation as a key limitation in model performance. To address this, we introduce strategies for densification including blur split and depth reinitialization, and simplification through intersection preserving and sampling. These techniques reorganize the spatial positions of the Gaussians, resulting in significant improvements across various datasets and benchmarks in terms of rendering quality, resource consumption, and storage compression. Our Mini-Splatting integrates seamlessly with the original rasterization pipeline, providing a strong baseline for future research in Gaussian-Splatting-based works. \href{https://github.com/fatPeter/mini-splatting}{Code is available}.

==> chapters/050_discussion.tex <==





% \begin{figure*}[h]
% 	\centering
% 	\includegraphics[width=1\linewidth]{figures/exp/limitation.pdf}
%     % \vspace{-0.7cm}
%     \caption{Ablation studies. (a): Ablation study on the importance-based feature and entropy encoding. (b): Ablation study on each component of our framework.}
% 	\label{fig:abl}
% \end{figure*}







% \noindent\textbf{Limitation.}



% \noindent\textbf{Future work.}












==> tables/storage.tex <==



\begin{table*}[]
    \renewcommand{\tabcolsep}{1pt}
    \centering
    \caption{Quant}
    \label{tab:storage} 
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{@{}l@{\,\,}|cccc|cccc|cccc}
    Dataset & \multicolumn{4}{c|}{Mip-NeRF 360} & \multicolumn{4}{c|}{Tanks\&Temples} & \multicolumn{4}{c}{Deep Blending}  \\
    
  Method $|$ Metric & SSIM $\uparrow$ & PSNR $\uparrow$ & LPIPS $\downarrow$ & Storage   & SSIM $\uparrow$ & PSNR $\uparrow$ & LPIPS $\downarrow$ & Storage   & SSIM $\uparrow$ & PSNR $\uparrow$ & LPIPS $\downarrow$ & Storage \\\hline


    3DGS~\cite{kerbl20233d}  & 0.815  & 27.47  & 0.216  & 792.56  & 0.848  & 23.66  & 0.176  & 434.97  & 0.904  & 29.54  & 0.244  & 666.07  \\
    Niedermayr \etal~\cite{niedermayr2023compressed} & 0.801  & 26.98  & 0.238  & 28.80  & 0.832  & 23.34  & 0.194  & 17.28  & 0.898  & 29.38  & 0.253  & 25.30  \\
    Lee \etal~\cite{lee2023compact} & 0.797  & 27.03  & 0.247  & 29.10  & 0.831  & 23.32  & 0.202  & 20.90  & 0.900  & 29.73  & 0.258  & 23.80  \\ \hline
    Mini-Splatting-C & 0.820  & 27.17  & 0.219  & 26.65  & 0.844  & 23.30  & 0.183  & 16.51  & 0.911  & 29.96  & 0.240  & 26.52  \\
    \end{tabular}
    }
    \vspace{-0.1in}
\end{table*}








